Nature and statistical properties of quasar associated absorption systems in the XQ-100 Legacy Survey

We statistically study the physical properties of a sample of narrow absorption line (NAL) systems looking for empirical evidences to distinguish between intrinsic and intervening NALs without taking into account any a priori definition or velocity cut-off. We analyze the spectra of 100 quasars with 3.5 < z$\rm_{em}$ < 4.5, observed with X-shooter/VLT in the context of the XQ-100 Legacy Survey. We detect a $\sim$ 8 $\sigma$ excess in the number density of absorbers within 10,000 km/s of the quasar emission redshift with respect to the random occurrence of NALs. This excess does not show a dependence on the quasar bolometric luminosity and it is not due to the redshift evolution of NALs. It extends far beyond the standard 5000 km/s cut-off traditionally defined for associated absorption lines. We propose to modify this definition, extending the threshold to 10,000 km/s when also weak absorbers (equivalent width < 0.2 \AA) are considered. We infer NV is the ion that better traces the effects of the quasar ionization field, offering the best statistical tool to identify intrinsic systems. Following this criterion we estimate that the fraction of quasars in our sample hosting an intrinsic NAL system is 33 percent. Lastly, we compare the properties of the material along the quasar line of sight, derived from our sample, with results based on close quasar pairs investigating the transverse direction. We find a deficiency of cool gas (traced by CII) along the line of sight associated with the quasar host galaxy, in contrast with what is observed in the transverse direction.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
